Identifying Vulnerable Third-Party Java Libraries from Textual Descriptions of Vulnerabilities and Libraries

To address security vulnerabilities arising from third-party libraries, security researchers maintain databases monitoring and curating vulnerability reports. Application developers can identify vulnerable libraries by directly querying the databases with their used libraries. However, the querying results of vulnerable libraries are not reliable due to the incompleteness of vulnerability reports. Thus, current approaches model the task of identifying vulnerable libraries as a named-entity-recognition (NER) task or an extreme multi-label learning (XML) task. These approaches suffer from highly inaccurate results in identifying vulnerable libraries with complex and similar names, e.g., Java libraries. To address these limitations, in this paper, we propose VulLibMiner, the first to identify vulnerable libraries from textual descriptions of both vulnerabilities and libraries, together with VulLib, a Java vulnerability dataset with their affected libraries. VulLibMiner consists of a TF-IDF matcher to efficiently screen out a small set of candidate libraries and a BERT-FNN model to identify vulnerable libraries from these candidates effectively. We evaluate VulLibMiner using four state-of-the-art/practice approaches of identifying vulnerable libraries on both their dataset named VeraJava and our VulLib dataset. Our evaluation results show that VulLibMiner can effectively identify vulnerable libraries with an average F1 score of 0.657 while the state-of-the-art/practice approaches achieve only 0.521.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> backup/ICSE_response.tex <==
【意见汇总】Topk的意见是什么
Review1：1.关于Chronos，我们的claim不准确（我们的motivation）
Reviewer2：1.方法过于直接（应该从motivation讲清楚，现有方法哪里不行） 2.我们的效果看起来不高（metric和效率）
Reviewer3：1.motivation不足（为什么不用NER approach，他们效果看起来不错）；2.我们的效果看起来不高

【Motivation的不足】
Reviewer1: Chronos也提出并尝试解决了zero-shot的问题
"VulLibMiner is not the only approach that can identify zero-shot libraries - Chronos targets this problem, too"
Reviewer2: 方法过于直接（我们的动机不明确，现有方法根本上哪里不足）
"The method outlined in the "Approach" section appears to be overly straightforward."
Reviewer3: 为什么不直接用NER approach，他们效果看起来不错
"Furthermore, one can argue that it is a trivial task to simply go over the vulnerability description, find the library name, and fill it into the label field in the report. The authors should provide a stronger motivation for the current problem setup."

【motivation的改进】
任务用途：是否需要从SCA的角度来说：对SCA工具来说，他们最关心的是直接被漏洞影响的包（核心问题），所以我们要解决这个问题

Identify vulnerable Java library的难点：包数量多且包名复杂（我们注意到现有方法在Java上表现很差）
1. 同样一个包有很多别名（的entity），或者很多包同一个别名（的entity）（比如group id相同/artifact id相同）
2. 大量没有被漏洞影响过的包/很少被影响过的（zero/few-shot的场景）
现有方法的局限性：
-> XML-based: 1.在Java场景上效果差；2.只能在top1000的包里做分类；3.实际需求要考虑更多的包，如果用全部的Java包进行映射，效果会更差（原因2）
-> NER-based: 是一个解决的思路，虽然识别entity已经很准确了（F1=90%），在Java上仍不能找出对应的包（F1=15%）（原因1）
   我们基于现有NER的方法设计两个直接的baselines：
    -> 只基于NER检索的结果做匹配
    -> 基于NER检索的结果，然后只考虑频率最高（训练集里出现过的, i.e., non-zero-shot）的包
通过实验【RQ1，可以开源】标明，以上两类方法在Java上准确率都不高，zero-shot场景下都更低

我们提出：加上包描述可以解决这两个问题

【事实性的错误】
Reviewer1：为什么Chronos效果下降了这么多
"I have, however, a major issue with the results reported for Chronos. Why do the values for R, P, and F1-score of Chronos differ so much from the original paper?"

【事实性错误的改进】
在motivation里增加一个empirical study：说明Chronos在Java上效果就会有很大的下降，在zero-shot上效果进一步下降（全部包而不是top1000）

----------------------------------------------------------------------------------------------------------------------
【实验的不足】
Reviewer1: 预排序没说清楚（动机、效果）
The motivation of the second idea, i.e., using a pre-screening stage, is not fully convincing to me. In my opinion, it is only needed when a user wants to classify a huge amount of libraries. And even in such a scenario, the user might consider to parallelize the classification or do it incrementally. I do not think that a user wants to classify all possible combinations of libraries and vulnerabilities at once. This argument should be down-tuned.

Reviewer2：缺少对false-positive/negative的分析；总体F1不高，效率没有baseline快
"The paper lacks an in-depth analysis of the false-positive and false-negative cases observed during the experimental phase.
While the proposed algorithm has been evaluated, the overall accuracy appears to fall short in adequately tackling the labor-intensive challenge of mapping CVEs to libraries.
The efficiency concern highlighted as a challenge is not satisfactorily addressed based on the comparative outcomes presented."

Reviewer3: 总体F1不高，需要和NER方法比较；缺少对false-positive/negative的分析
"precision and recall are low, which limits the utility of the proposed approach
missing comparison baselines and related work
The assumption on the similarity between a vulnerability description and a library description does not always hold, which may explain the low precision and recall
A lack of analysis of the cases that VulLibMiner fails to identify"

【实验的改进】
1.修改metrics
- 和Chronos的metric保持一致，也避免了F1@k上限不是1的问题
- F1可以从0.56提升到0.64
2.修改实验setup
- 预排序阶段默认保留从Top128改为Top256，预计提升F1到0.74
- 效率不和baseline相比，只说明我们可以200ms识别一个漏洞影响的包【可以接受】
3.调整预排序的RQ【对应challenge里效率和准确率的权衡】
- 实验内容: 预排序保留Top128，Top256，Top512，Top1024，Top300,000，看我们方法的整体准确率和效率
- 实验目的：说明预排序本身是有意义的，在几乎不损失准确率的前提下，效率提升非常大（1000倍）
4.完善case study：
我们的逻辑是：
- 对于包名可以区分的（简单的case），我们可以通过<漏洞描述，包名>做监督学习
- 包名差别不那么大的情形（SOTA解决的不好的），但是描述差别比较大的，加入描述后基于entity-linking的可以显著增强
- 如果都相差不大，那就是false positive/negative，那就需要更多的信息去区分这两个包
因此，case study应该选取一个都相差不大的例子

【其他的意见】
数据集细节：
Reviewer1：负样本意义不明；标注过程中冲突怎么办
"The usage of negative samples is not fully clear to me. In general, it is a good idea to also include negative samples, however why using negative samples from other programming languages and not Java? It does not sound practical to me to identify a C++ vulnerability in a Java library. In my opinion, it would be more practical to add Java libraries that do not suffer from any vulnerability as negative examples, for instance by adding pairs <NO_CVE, JavaLib>?
Regarding the manual effort to create the datasets, I was wandering whether there was lots of discussion and agreement or disagreement between the software engineers, in particular when double checking the labels in the datasets?"
Reviewer2：标注的时候ground truth怎么定的
"The author pays additional attention to ensuring dataset fairness in comparison with other tools. Nevertheless, the absence of explanations regarding the establishment of a ground truth standard and the limited elaboration on the analysis of false cases impact the rigor of the paper."

解决方案：
- 去掉负样本，这本来就是一个分类问题
- 加上标注细节，两个人冲突怎么办，找第三个人评审，（还不明确的直接搁置，不收入数据集？）

代码开源：
Reviewer1：代码没开源
"The submission provides a replication package that contains the two datasets, however misses the source code. As a reason the replication packages mentions the security requirements of their industrial partner. This is unfortunate because without the source code it is difficult to replicate the studies and check the validity of the results."

Reviewer3: 代码没开源，缺少部分数据
"The code of VulLibMiner is not provided, and the provided VeraJava dataset does not include the description of CVEs and libraries."

解决方案：
- 加一句：我们可以帮忙跑对比实验；把predict score也放出去；把baseline的代码放出去
- 咨询一下老师，没有code重不重要；如果重要，没有code怎么圆比较好
- 将VeraJava的数据【描述】补上

【最后一个问题：投S&P(12.06)还是期刊TSE/TOSEM/TDSC】

## Major Revision Idea

Add two motivation research questions to illustrate the difficulty of identifying Java libraries.
[就用公开数据集整体做一个对比；再在java上进一步做一个对比]

Background:
1) Task Formalization: identify vulnerable library, two definitions of zero-shot identification

2) Then explain the limitations of existing approaches
-> XML-based: library name entity tokens != library name, especially Java libraries, using evaluation results
-> NER-based: zero-shot identification (especially from 300,000 ones instead of 1,000 ones), using examples (using TF-IDF)
 
Evaluation:
Change evaluation metrics:
1) The ground truth of our evaluation metrics (F1@k, k=1,2,3) is 0.867, 0.931, and 9.840, respectively.
-> modify the denominator of precision@k from k to min(k, label) (the same as Chronos).
-> Thus, our F1 can increase from 0.56 to 0.64 (finished)

Change evaluation setups:
1) 0.561 is the result of reranking on Top 128 (recall@128 = 0.75), using Top 256 instead (recall256=0.85, thus F1@3 is approximated to achieve 0.7 or higher)
-> checkpoint path: bucket-5650/lilin/soft_auto_mapping/output_yundao/multi-label-combine-negative-128/BertFNNSimple_checkpoint/
-> Thus, our F1 can increase from 0.64 to 0.74 (approximately)

Add discussions:
1) how to use the identified results: 
-> for simple results (or can be double confirmed), do not depend on manual efforts
-> engineers need to select choices instead of fill-in-the-blanks

2) indirectly affected libraries:
-> we have already used both names and descriptions; 
-> as for those indirectly affected libraries (no dependency in both name and descriptions), mainly due to their indirect dependencies, we can use existing approaches to identify them based on their dependencies




Review #127A
===========================================================================

Overall merit
-------------
1. Reject

Overall Comments for authors
----------------------------
The paper addresses a relevant problem and also presents two novel ideas for improving the identification of vulnerable third party libraries. Among the two novel ideas, particular the idea of using the library description(s) instead of only the package name(s), sounds promising. 
[Strength]

The evaluation, however, misses a detailed treatment of existing baseline approaches, most prominently Chronos. Because of the rather large differences in the performance reported in the original Chronos paper and this submission, the validity of the presented results is questionable. Also the claim that existing approaches do not identify zero-shot libraries needs to be down-tuned since, in particular Chronos, is addressing this problem, too.
[Weakness]

Strengths
---------
+ promising idea to use the library descriptions instead of only package names for vulnerability identification

Weaknesses
----------
- VulLibMiner is not the only approach that can identify zero-shot libraries - Chronos targets this problem, too
[Chronos identify vulnerable libraries from only vulnerable libraries, i.e., 2000 ones; while we focus on identifying libraries from all libraries][clarify the definition][搞清楚zestXML的zero-shot能力的来源]

- differences in the performance values reported in the original Chronos paper and this submission lack an explanation
[We extract Java libraries from all libraries, which explains their drop in effectiveness.]

- the impact of the pre-screening stage on the performance of VulLibMiner is questionable since only the recall is reported
[add precision results, actually we focus on recall because we will conduct re-order on its results]
[the precision results only reflect their ineffectiveness]
- replication package is provided but misses the source code to replicate the studies
[加一句：我们可以帮忙跑对比实验；把predict score也放出去]

Comments on Rigor
-----------------
The VulLibMiner approach is well described in Section 3. I only have one question regarding the FNN: did you try to feed the output of the BERT model into a traditional machine learning algorithm, such as Random Forests or SVM, for the classification of vulnerabilities?

[No, we just add one layer;]

Regarding the datasets presented in Section 4, also Chronos is providing their dataset. The GitHub repo (https://github.com/soarsmu/Chronos/tree/main) shows that its dataset was made available 6 months ago and therefore could have been considered. Why was it not considered? Also, because the performance of Chronos reported in the original paper significantly differs from the performance reported in this submission. 

[They use the same dataset as FastXML or LightXML, actually we use this dataset]
[还是得解释清楚为什么要裁出Java来：“整体的结果已经还可以了，但是我们发现它Java的效果很差”]

The usage of negative samples is not fully clear to me. In general, it is a good idea to also include negative samples, however why using negative samples from other programming languages and not Java? It does not sound practical to me to identify a C++ vulnerability in a Java library. In my opinion, it would be more practical to add Java libraries that do not suffer from any vulnerability as negative examples, for instance by adding pairs <NO_CVE, JavaLib>?

[our task identify vulnerbility -> Java lib, so it should output the class "no Java Lib" (in short, negative sample)]
[Maybe it's better to use another name instead of negative sample]
[去掉负样本，这本来就是一个分类任务，不需要负样本]

Regarding the manual effort to create the datasets, I was wandering whether there was lots of discussion and agreement or disagreement between the software engineers, in particular when double checking the labels in the datasets?

[add more details, we require the third engineer to address disagreement]

The evaluation is reported in Section 5. The general setup for the evaluation is OK: two datasets are used and the results are compared with four baseline approaches based on P, R, and F1-score.
I have, however, a major issue with the results reported for Chronos. Why do the values for R, P, and F1-score of Chronos differ so much from the original paper? The Chronos paper reports an F1@1 score of 0.67 compared to 0.437 and 0.360 in this paper. Also the values of LightXML (which was evaluated in both papers) differ, though in this paper were higher than in the Chronos paper. What is the reason for these differences? Without a detailed explanation of these differences, the 
validity of the results is questionable. 

[That's its reported results in Java, we simple focus on Java results].
[拿全量数据比一次，全量会不会效果下降]

Furthermore, regarding identifying zero-shot libraries, Table 4 shows zeros for FastXML, LightXML and Chronos for the VulLib dataset. What is the reason for that? Also, is there a  difference between the results from RQ1 and the full-shot set in RQ2? Is the full-shot testing set not the same dataset as used in RQ1?
[他们不支持从300,000里找出来收影响的][在RQ1里加一个29%的zero-shot（真实场景的比例）]
[Totally different, the results in RQ1 contain 29% zero-shot libraries, which follows the distribution in the real world]

The method for evaluating the effectiveness of the TF-IDF matcher is not fully clear to me. In particular, why was only the recall evaluated? Why not performing an ablation study in which the TF-IDF matching stage is skipped? In this way, the effect of the TF-IDF matching on the performance of VulLibMiner could be assessed more accurately. 

[TF-IDF only filters irrelavent libraries, so recall is important, whether it removes vulnerable libraries. Also, we can add precisions][Figure 3 加一个解释Y轴]

Regarding RQ4, the average time for classifying a library is 203 ms which is higher than existing approaches. For instance, Chronos's prediction is almost 2x faster than VulLibMiner. Regarding the total time to predict all vulnerabilities for all Java libraries, the authors should consider that this will rarely happen. Instead, engineers will more likely use such an approach to predict the vulnerabilities for the libraries that they plan to use in their project. Furthermore, each library will most likely be classified only once so that classification will most likely happen incrementally. Finally, the classification can be parallelized, for instance on multiple machines, which will also help to reduce the total time significantly.

[Maybe we can remove the efficiency of baseline approaches, as 200ms is already highly efficient.]

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
In general, identifying vulnerable third party libraries is a relevant research topic. That is also one reason, why many approaches were proposed in the past. VulLibMiner aims to improve over existing approaches and also considers to identify vulnerable zero-shot libraries. In this regard, the shortcomings of several existing approaches are discussed in the introduction, however, one important one is missing, namely Chronos. Chronos specifically addresses the challenge of identifying zero-shot libraries and it remains unclear to me which gaps remain that VulLibMiner aims to fill. What are the shortcomings of Chronos that VulLibMiner aims to address? Without a thorough discussion of the shortcomings of Chronos and differences to it the relevance of novel contributions presented in this paper are unclear to me. 

Furthermore, as mentioned above, the values of the performance metrics reported for Chronos deviate significantly from the values reported in the Chronos paper [25]. [25] reports an F1@1 score of 0.67 and an avg. F1 score of 0.75 while the given paper reports an F1@1 score of 0.437 and 0.360 for VeraJava and VulLib. Without a detailed discussion of these difference(s) the claimed improvements over Chronos are unclear to me.

[
    Add two motivation research questions:
    1. the difficulty of identifying Java libraries.
    -> Java libraries are difficult
    2. the difference of two definitions of zero-shot libraries [from 1,000 and 300,000 libraries]
    -> Baselines' effectiveness on two levels of zero-shot libraries
    -> real zero-shot (identifying vulnerable libraries from 300,000 ones) is necessary & difficult
]

Comments on Novelty
-------------------
The two main novel ideas of VulLibMiner are 1) using the library description instead of only the library (package) name, and 2) pre-screening potential vulnerable libraries using a TF-IDF technique. In particular the first idea sounds interesting to me and is well motivated and explained in the paper. The motivation of the second idea, i.e., using a pre-screening stage, is not fully convincing to me. In my opinion, it is only needed when a user wants to classify a huge amount of libraries. And even in such a scenario, the user might consider to parallelize the classification or do it incrementally. I do not think that a user wants to classify all possible combinations of libraries and vulnerabilities at once. This argument should be down-tuned.
[200ms -> 5min，也很慢了；benchmark全跑一遍，需要接近两天；1）加一个ablation study，只看BERT的效果；2）128已经拿到所有的recall了，性能最多折损10%]

Comments on Verifiability and Transparency
------------------------------------------
The submission provides a replication package that contains the two datasets, however misses the source code. As a reason the replication packages mentions the security requirements of their industrial partner. This is unfortunate because without the source code it is difficult to replicate the studies and check the validity of the results.

Comments on Presentation
------------------------
Overall the paper is well written and makes good use of figures and tables. I only found a few typos plus some issues with the number of subsections. See below for more details.

l187 (and other places): the numbering 2.0.x is unusual. Introduce a subsection 2.1 and then use 2.1.x.
l324: The process .. is shown in Figure 1.
l446: ... model that accurately identifies ...
l513: ... practical challenges ...
l622: please remove "Veracode".

[fix them]



Review #127B
===========================================================================

Overall merit
-------------
2. Weak reject

Overall Comments for authors
----------------------------
There are some aspects should be improved:

### Originality (Novelty)

- The concept of incorporating the library description is intriguing and innovative.

### Soundness:

Following concern should be addressed: 

- Dataset Construction: The paper should establish a foundational standard for validating the correctness of CVE-to-Java-library mappings. Presently, the paper lacks comprehensive insights into the specific steps undertaken to verify the alignment between CVEs and Java libraries.

[add more details, we require the third engineer to address disagreement]

- Issue Highlight: The findings provided in Table 5 indicate that the algorithm developed does not adequately address the efficiency issue as indicated.

[remove baselines' efficiency, 200ms per vulnerability is already highly efficient]
[或者加一个ablation study，只看BERT的效果；2）recall@128已经包括差不多所有labels了，性能最多折损10%]

- Pertinence of Related Works: It is important to mention that SCA tools like ATVHunter appear to be unrelated within the context of this paper.
[已经提到了，举得例子就是它]

### Significance

- Due to the insufficient level of soundness, the extent of significance remains constrained.

Strengths
---------
+ The research problem addressed in the paper holds practical significance.
+ The proposed algorithm is clearly explained and evaluated using diverse datasets.

Weaknesses
----------
- The method outlined in the "Approach" section appears to be overly straightforward.
[need discussion]
- The paper lacks an in-depth analysis of the false-positive and false-negative cases observed during the experimental phase.
[其实是F1不够高的原因，调整metrics和evaluation setup]
- While the proposed algorithm has been evaluated, the overall accuracy appears to fall short in adequately tackling the labor-intensive challenge of mapping CVEs to libraries.
[同上]
- The efficiency concern highlighted as a challenge is not satisfactorily addressed based on the comparative outcomes presented.
[the same as the preceding results]

Artifact Assessment
-------------------
4. Good (largely as promised)

Comments on Rigor
-----------------
The author pays additional attention to ensuring dataset fairness in comparison with other tools. Nevertheless, the absence of explanations regarding the establishment of a ground truth standard and the limited elaboration on the analysis of false cases impact the rigor of the paper.
[add the details of manually labelling, e.g., engineers can label them based on recommended libraries instead of manually searching]
[加上标注细节，两个人冲突怎么办]

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
The subject matter revolves around a noteworthy issue within the software engineering community, and the associated techniques also hold importance in the realm of software engineering.

Comments on Novelty
-------------------
The concept introduces a fresh perspective by utilizing library descriptions for CVE mapping. In contrast, existing state-of-the-art methods rely on simplistic features such as library names, which can result in both high false positives and false negatives.

Comments on Verifiability and Transparency
------------------------------------------
The provided dataset is accessible and corresponds to the depiction provided in the paper, thus contributing to the verifiability and transparency of the research findings.

Comments on Presentation
------------------------
Certain segments of the writing display a degree of confusion and would benefit from improvements to enhance clarity and comprehension.

- In Section 2,  "The objective ... libraries that are affected by a particular CVE description." -> affected by description ?
- Table 3 in Section 5.4.3 contains duplicated names within the two rows of the Dataset section, which requires correction. 
- In Section 5.3, there seems to be no imperative requirement for the inclusion of formulas pertaining to precision, recall, and F1-score.

[fix them]




Review #127C
===========================================================================

Overall merit
-------------
2. Weak reject

Overall Comments for authors
----------------------------
This work addresses a relevant problem to SE and the proposed approach seems novel. However, I have several concerns regarding the motivation, approach, and evaluation. 

*Motivation* 
this work focuses on recognizing library names in a vulnerability report. Compared with other kinds of online text documents such as Tweets and Stack Overflow posts, which are more informal and involve more ambiguity, vulnerability reports sound easier to process given their formality. Thus, it could be more challenging and technically interesting to recognize vulnerable libraries mentioned in informal text descriptions. Furthermore, one can argue that it is a trivial task to simply go over the vulnerability description, find the library name, and fill it into the label field in the report. The authors should provide a stronger motivation for the current problem setup.

[focusing on the difficulty of Java vulnerability && zero-shot ones]
[还是要讲透: library name entity tokens != library name，所以NER approaches F1不够]
[加一个trivial的baseline，只基于NER检索的结果做匹配，只考虑2000个包的别名；再做一个trivial的baseline，只考虑频率最高（训练集里有的）的包]
[可能会提到不相关的包，同样一个包的别名是不是很多，或者很多包同一个别名（不同group id/不同的artifact id）；我们没有见过的包（很少见过的）]
[VIEM只是区分和CPE是否一致]

*Approach*
In this work, the authors formulated the library identification problem as a text-matching problem rather than a token classification problem in a typical NER setting. Instead of matching a vulnerability description with a bunch of library names, the authors could simply run an NER model that detects library entities mentioned in the vulnerability description. There have been quite a few existing approaches for recognizing library and API names in software documents [1,2,3,4]. Most recent approaches can achieve over 80% precision and recall on library detection. Why not use these approaches?

1. Ye, Deheng, Zhenchang Xing, Chee Yong Foo, Zi Qun Ang, Jing Li, and Nachiket Kapre. "Software-specific named entity recognition in software engineering social content." In 2016 IEEE 23rd international conference on software analysis, evolution, and reengineering (SANER), vol. 1, pp. 90-101. IEEE, 2016.
2. Tabassum, Jeniya, Mounica Maddela, Wei Xu, and Alan Ritter. "Code and Named Entity Recognition in StackOverflow." In Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics, pp. 4913-4926. 2020.
3. Zhang, Ting, Divya Prabha Chandrasekaran, Ferdian Thung, and David Lo. "Benchmarking library recognition in tweets." In Proceedings of the 30th IEEE/ACM International Conference on Program Comprehension, pp. 343-353. 2022.
4. Nguyen, Tai, Yifeng Di, Joohan Lee, Muhao Chen, and Tianyi Zhang. "Software Entity Recognition with Noise-Robust Learning." In 2023 38th IEEE/ACM International Conference on Automated Software Engineering (ASE), pp. 1-12. IEEE, 2023.

[Do not mention text-matching, using entity-linking instead, and then use TF-IDF to illustrate that library name entity tokens != library name]
[Even if 0.9 accuracy of NER cannot lead to a high identification accuracy (identifying Java library)]

Furthermore, the proposed approach assumes that there are some overlaps between a vulnerability description and a library description. However, this assumption may not hold for many libraries and vulnerabilities. For example, the Log4j vulnerability (CVE-2021-44228) affects many libraries whose description is not similar to the description of this vulnerability, because Log4j is widely used by diverse projects. Based on the VulLibMiner approach, these libraries are excluded by the TF-IDF algorithm in the screening step. This issue can be one possible reason for the low precision and recall of the proposed approach.
[including both names and descriptions; as for those indirectly affected libraries, add into discussion: we can use other approaches to identify them based on their dependencies (existing work)]
[对SCA工具来说，他们最关心的是直接影响的漏洞（核心问题），我们只关心这个问题；他们也会通过依赖分析得到间接影响的包]

Related to the first concern, it will be helpful to quantify how many libraries in the datasets have similar descriptions with the vulnerability and how many libraries do not have similar descriptions. In RQ3, the recall on VulLib dataset can only reach 0.9 even when the Candidate Library Size is as high as 1024. 

[ground truth的描述和漏洞描述没有交集；还有一个可能是所有包的描述都差不多-> 这两个原因导致recall不够高]
[强调1000/300,000，比如功能相同的包（artifactid相同的情形）]
[对于这种描述相同的，我们可以通过包名做监督学习，对于包名差别不那么大的情形，但是描述差别比较大的，基于entity-linking的可以显著增强；如果都相差不大，那就是false positive/negative，那就需要更多的信息去区分这两个包]
[make some empirical study]

*Evaluation*

The authors only used a TF-IDF matching method as the comparison baseline from the line of NER models. However, this TF-IDF method is not a typical NER model. The authors should choose a state-of-the-art NER model that is developed for recognizing libraries, like one of the four papers above. As mentioned earlier, those models can achieve over 80% precision and recall when detecting library names in informal text, which stands as a stronger baseline. It is also not clear why not choose VIEM [10] as a baseline.
[那就focus on Java的场景，因为Java的entity，Java里xxx%的token就是不一致的，即使用这些token去搜，效果也不会太好]
[VIEM不是baseline，要说清楚]

Since the proposed approach only achieves 60%-70% precision and around 50% recall, the authors should do an in-depth analysis of the misclassified cases to understand why the precision and recall are so low. I am also a bit concerned about how useful this approach is in practice. 

[change our evaluation metrics and evaluation setup]

Furthermore, in section 5.7.2, the time consumption for FastXML to identify a vulnerable library is 9.7 ms, which is faster than the TF-IDF used by VulLibMiner. Given the precision and recall of FastXML Full-Shot samples are rather high, is it possible to replace TF-IDF with FastXML? It's better to include an ablation study to compare the effectiveness of TF-IDF and FastXML.

[FastXML没有zero-shot能力，所以会把zero-shot的包排除掉（我们希望把答案都留下）]
[recall@128不够高] [不用提fastxml的效率]
[do not compare efficiency with baselines, 0.2ms is efficient enough]

In RQ1, the precision of VulLibMiner decreases significantly when k increases, it's better to analyze the cases that VulLibMiner identifies incorrectly.

[很多漏洞影响的包数量 <k，所以我们把precision的分母换成min(k, num)]
[this issue can be addressed by new metrics]

Finally, the code of VulLibMiner is not provided, and the provided VeraJava dataset does not include the description of CVEs and libraries.

[The descriptions is used for both datasets, make another csv file]
[咨询一下老师，没有code重不重要；如果重要，没有code怎么圆比较好]

Strengths
---------
- A novel idea
- A comparison with multiple baselines on two datasets and a subset of zero-shot library names

Weaknesses
----------
- weak motivation
[using the revised motivation: Java & real zero-shot]
- precision and recall are low, which limits the utility of the proposed approach
[using the modified metrics and top256 filtered results (instead of top 128), thus achieving 0.7]
- missing comparison baselines and related work
[Do not mention text-matching, using entity-linking instead, and then use TF-IDF (with a NER model) to illustrate that library name entity tokens != library name]
[Even if 0.9 accuracy of NER cannot lead to a high identification accuracy (identifying Java library)]
- The assumption on the similarity between a vulnerability description and a library description does not always hold, which may explain the low precision and recall
[change our evaluation metrics and evaluation setup to improve our F1 to ~0.73]
- A lack of analysis of the cases that VulLibMiner fails to identify
[specify our case study]
- Incomplete artifacts

Comments on Rigor
-----------------
As mentioned in the overall comments, this work suffers from several rigor issues. The assumption of the similarity between vulnerability descriptions and library descriptions may not hold in practice. There is also a typical alternative approach not considered in the design and evaluation. 
[mainly due to low metric scores]

One issue not mentioned above is the data labeling procedure. It is not clear how the labeling tasks were distributed to the 10 data labelers. Evenly distributed? Or did each labeler work independently on all tasks and use the majority vote as the final label?
[clarify them, the same as preceding]

Another potential issue is that VulLib includes way fewer negative samples compared with possible samples (Figure 2). So it is essentially an imbalanced dataset. It is unclear what kind of impact this data balance issue may have on the evaluation results.
[remove negative samples, this is a classification task indeed]

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
Vulnerable library identification is a relevant SE problem.

Comments on Novelty
-------------------
To the best of my knowledge, this work is the first to consider the descriptions of libraries to detect vulnerable libraries mentioned in a vulnerable report.

Comments on Verifiability and Transparency
------------------------------------------
The code of VulLibMiner is not provided, and the provided VeraJava dataset does not include the description of CVEs and libraries.

Comments on Presentation
------------------------
The presentation is clear overall, but there are some issues:

In Line 178-179, "The aim of identifying vulnerable libraries is to extract the package name displayed in the Label field" is misleading. It sounds like the goal is to extract the lib name from the CPE field, which already exists in the example. But I think what it really means is to extract the library name from the description and then fill it in. 

In Listing 2, the output of the first two parts is both marked as "Output of Existing approaches". It should be distinguished that the first part is the output of NER-based approaches and the second part is the output of XML-based approaches.

In Section 3.1.1, it mentions the tags for tokens: "[NN, NNS, NNP, NNPS, JJ, JJR, JJS]"(line 377-378), it is better to clarify their meanings.

In Table 3, the two entries in "Dataset" column should be "VeraJava" and "VulLib", but they are both "VeraJava".

In Section 4.0.2, there is a lack of description of "our own vulnerability database."

The study in RQ3 is not really an ablation study since the TF-IDE method is not ablated. Instead, it sounds more like a sensitivity analysis of the candidate size k.

[fixes them]




















































<!--
2) the difference of two levels of zero-shot libraries
- Baselines' effectiveness on two levels of zero-shot libraries
-> real zero-shot (identifying vulnerable libraries from 300,000 ones instead of 1,000 ones) is necessary & difficult
 -->


==> tables/chronos.tex <==
raw:

K = 1
P@1 =  0.5167785234899329
R@1 =  0.3783277768019168
F@1 =  0.43684570162711805
K = 2
P@2 =  0.41387024608501116
R@2 =  0.5716129705104737
F@2 =  0.48011695539135957
K = 3
P@3 =  0.32065622669649513
R@3 =  0.6417247529668546
F@3 =  0.4276332184704512
K = 100
P@100 =  0.025436241610738073
R@100 =  0.9116172316175021
F@100 =  0.0494915537318263

full-shot
K = 1
P@1 =  0.5346820809248555
R@1 =  0.3755660392017056
F@1 =  0.4412169098182886
K = 2
P@2 =  0.42485549132947975
R@2 =  0.5482013424417584
F@2 =  0.47871068288561863
K = 3
P@3 =  0.34007707129094333
R@3 =  0.6297382257648716
F@3 =  0.44165014131705754
K = 100
P@100 =  0.029537572254335096
R@100 =  0.8949698531782949
F@100 =  0.05718772175644776


In [147]: len(java_test_full)
Out[147]: 101

In [148]: len(java_test_zero)
Out[148]: 346

In [149]: len(java_test_index)
Out[149]: 447


==> tables/comments.tex <==
 e.g., what is the demographic of the two senior software engineers? Are they experts in security vulnerability? What criteria are applied to mapping the dataset's <CVE, lib> pairs? To what extent do they have conflicts during labeling, and how do they resolve them? Moreover, when going through the provided 255 <CVE, lib> pairs, the correctness is greatly raising my concerns. 

 [Presentation] Some of the writing in the paper is unclear, making it difficult to comprehend the dataset construction details. For example, the paper claims in Section 1 and Section 4.2.2 that the VulLib dataset was manually labeled and validated by senior software engineers. However, the paper does not provide any information about the senior software engineers' backgrounds, such as their credibility and experience with Java. It is crucial for the authors to provide a detailed description for better reproducibility. Additionally, since these engineers are not the developers of the libraries, it is unclear how valid the dataset is. Moreover, the authors have not made their datasets publicly available, which makes it challenging to verify their findings.



##### An example of correctly identified libraries
`CVE-2022-2963` is an example vulnerability that VulLibMiner correctly recommand its affected libraries.
It is a SQL injection vulnerability whose description is listed as follows:

It is a memory leak bug of jasper whose description is listed as follows:
~~~
A vulnerability found in jasper. This security vulnerability happens because of a memory leak bug in function cmdopts_parse that can cause a crash or segmentation fault.
~~~

However, NVD only includes `cpe:2.3:a:jasper_project:jasper:3.0.6:` as its affected CPE, along with `fedora` and `linux`.
VulLibMiner recommand two `jasper-compiler` libraries that also includes the vulnerable function `cmdopts_parse`.

~~~
maven:jetty:jasper-compiler
maven:tomcat:jasper-compiler
maven:tomcat:jasper
~~~

##### An example of incorrectly identified libraries
`CVE-2022-3471` is an example vulnerability that VulLibMiner incorrectly recommand its affected libraries.
It is a SQL injection vulnerability whose description is listed as follows:
```
A vulnerability was found in SourceCodester Human Resource Management System. It has been declared as critical. Affected by this vulnerability is an unknown functionality of the file city.php. The manipulation of the argument searccity leads to sql injection. The attack can be launched remotely. The exploit has been disclosed to the public and may be used. The associated identifier of this vulnerability is VDB-210715.
```
Actually, it is a php vulnerability because `SourceCodester Human Resource Management System` is written in php.
However, the description of this vulnerability does not clearly tell the affected system and how this vulnerability is utilized.
Thus, VulLibMiner outputs some sql libraries and php libraries.
~~~
maven:org.apache.storm:sql
maven:cn.sexycode:my-sql
maven:dev.rudiments:sql
maven:xyz.cofe:sql
maven:taglibs:sql
maven:commons-sql:commons-sql
maven:org.cloudhoist:php
maven:cocoon:cocoon-php
~~~

![image.png](attachment:image.png)![image.png](attachment:image.png)




Jenkins Mac Plugin 1.1.0 and earlier does not validate SSH host keys when connecting agents created by the plugin, enabling man-in-the-middle attacks. What software is above sentence talking about?

maven:fr.edf.jenkins.plugins:mac

==> tables/eval.tex <==
1 64 0.6283185840707964 0.47994176914530895 0.5441976372261538
1 96 0.6637168141592921 0.5083622572118147 0.5757437122407606
1 128 0.7026548672566372 0.543907979925679 0.613173399637841
1 160 0.7115044247787611 0.5518725816955904 0.6216034988419943
1 192 0.7044247787610619 0.5470053250584223 0.6158140257443957
1 224 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 256 0.7150442477876107 0.5564448530820211 0.625853090105437
1 288 0.7150442477876107 0.5551174194537025 0.625012591490309
1 320 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 352 0.7150442477876107 0.5564448530820211 0.625853090105437
1 384 0.7185840707964601 0.5590997203386583 0.6288882363690067
1 416 0.7168141592920354 0.5582147645864458 0.6276504629624705
1 448 0.7168141592920354 0.5582147645864458 0.6276504629624705
1 480 0.7168141592920354 0.5582147645864458 0.6276504629624705
1 512 0.7150442477876107 0.5564448530820211 0.625853090105437
1 544 0.7115044247787611 0.5537899858253839 0.6228179339301624
1 576 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 608 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 640 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 672 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 704 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 736 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 768 0.7150442477876107 0.5564448530820211 0.625853090105437
1 800 0.7150442477876107 0.5564448530820211 0.625853090105437
1 832 0.7150442477876107 0.5564448530820211 0.625853090105437
1 864 0.7168141592920354 0.557034823583496 0.6269039016886445
1 896 0.7168141592920354 0.557034823583496 0.6269039016886445
1 928 0.7185840707964601 0.5588047350879207 0.6287015816485252
1 960 0.7185840707964601 0.5588047350879207 0.6287015816485252
1 992 0.7185840707964601 0.5588047350879207 0.6287015816485252
1 1024 0.7185840707964601 0.5588047350879207 0.6287015816485252
2 64 0.6115044247787611 0.5668633873501132 0.5883383202455638
2 96 0.6539823008849558 0.6059757499138031 0.6290644596586055
2 128 0.6964601769911505 0.6471683331417845 0.6709101041602659
2 160 0.715929203539823 0.6650283492318891 0.6895406965136408
2 192 0.7212389380530974 0.670043098494426 0.694699076266582
2 224 0.7309734513274336 0.6794826265180247 0.7042881638421795
2 256 0.7380530973451327 0.6873882312377887 0.7118202664265316
2 288 0.7415929203539823 0.6904855763705321 0.7151273009323443
2 320 0.7451327433628319 0.6940253993793816 0.7186716100812495
2 352 0.7451327433628319 0.6940253993793816 0.7186716100812495
2 384 0.7477876106194691 0.6966802666360188 0.7213298130842928
2 416 0.7495575221238938 0.6984501781404435 0.7231019348286224
2 448 0.7486725663716814 0.6975652223882312 0.7222158753089077
2 480 0.7495575221238938 0.6984501781404435 0.7231019348286224
2 512 0.7469026548672566 0.6957953108838064 0.7204437481448223
2 544 0.7460176991150442 0.694910355131594 0.7195576804804923
2 576 0.7424778761061946 0.6913705321227445 0.7160133823727665
2 608 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 640 0.7389380530973452 0.6881256943646323 0.7126272554879096
2 672 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 704 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 736 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 768 0.7380530973451327 0.6876832164885262 0.7119783974034849
2 800 0.7380530973451327 0.6876832164885262 0.7119783974034849
2 832 0.7380530973451327 0.6876832164885262 0.7119783974034849
2 864 0.7389380530973452 0.6882731869900011 0.7127063387790727
2 896 0.7407079646017699 0.6900430984944259 0.7144784751964081
2 928 0.7424778761061946 0.6918130099988506 0.7162506006315945
2 960 0.7424778761061946 0.6918130099988506 0.7162506006315945
2 992 0.7424778761061946 0.6918130099988506 0.7162506006315945
2 1024 0.7380530973451327 0.6873882312377887 0.7118202664265316
3 64 0.6227138643067849 0.6045625023943607 0.6135039544400294
3 96 0.6731563421828908 0.6533208826571657 0.6630903077800281
3 128 0.7197640117994101 0.6990570049419607 0.7092594039932004
3 160 0.7380530973451328 0.7159717273876567 0.7268447443558818
3 192 0.741297935103245 0.7195536911466117 0.7302639855523161
3 224 0.7513274336283189 0.7295831896716853 0.7402956760387077
3 256 0.7607669616519176 0.7392439566333373 0.7498510470182278
3 288 0.7651917404129795 0.7435212427690305 0.7542008587856368
3 320 0.768731563421829 0.7470610657778801 0.7577414086915233
3 352 0.7766961651917406 0.7550256675477917 0.765707621411733
3 384 0.7787610619469029 0.7570905643029539 0.7677729303659072
3 416 0.7823008849557525 0.7606303873118033 0.7713134548679701
3 448 0.7825958702064899 0.7609253725625409 0.771608498286004
3 480 0.7828908554572273 0.7612203578132782 0.7719035416595889
3 512 0.7820058997050148 0.7603354020610659 0.7710184114054363
3 544 0.7811209439528024 0.7594504463088535 0.7701332807503245
3 576 0.7820058997050148 0.7603354020610659 0.7710184114054363
3 608 0.7820058997050148 0.7603354020610659 0.7710184114054363
3 640 0.7805309734513275 0.7590079684327473 0.769619023385166
3 672 0.7787610619469026 0.7572380569283225 0.7678487651632744
3 704 0.7761061946902655 0.7545831896716854 0.7651933748236583
3 736 0.7761061946902655 0.7545831896716854 0.7651933748236583
3 768 0.7758112094395281 0.7545831896716854 0.7650499731858795
3 800 0.7764011799410031 0.7553206527985289 0.7657158545788109
3 832 0.7764011799410031 0.7553206527985289 0.7657158545788109
3 864 0.7761061946902655 0.7550256675477914 0.7654208134333593
3 896 0.776991150442478 0.7559106233000038 0.76630593674064
3 928 0.7778761061946904 0.7567955790522162 0.7671910596614435
3 960 0.7778761061946904 0.7567955790522162 0.7671910596614435
3 992 0.7761061946902655 0.7550256675477914 0.7654208134333593
3 1024 0.7758112094395281 0.7545831896716853 0.7650499731858795



1 64 0.6283185840707964 0.47994176914530895 0.5441976372261538
1 96 0.6637168141592921 0.5083622572118147 0.5757437122407606
1 128 0.7026548672566372 0.543907979925679 0.613173399637841
1 160 0.7115044247787611 0.5518725816955904 0.6216034988419943
1 192 0.7044247787610619 0.5470053250584223 0.6158140257443957
1 224 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 256 0.7150442477876107 0.5564448530820211 0.625853090105437
1 288 0.7150442477876107 0.5551174194537025 0.625012591490309
1 320 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 352 0.7150442477876107 0.5564448530820211 0.625853090105437
1 384 0.7185840707964601 0.5590997203386583 0.6288882363690067
1 416 0.7168141592920354 0.5582147645864458 0.6276504629624705
1 448 0.7168141592920354 0.5582147645864458 0.6276504629624705
1 480 0.7168141592920354 0.5582147645864458 0.6276504629624705
1 512 0.7150442477876107 0.5564448530820211 0.625853090105437
1 544 0.7115044247787611 0.5537899858253839 0.6228179339301624
1 576 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 608 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 640 0.7115044247787611 0.5529050300731715 0.6222578831088597
1 672 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 704 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 736 0.7132743362831858 0.5546749415775963 0.6240555639168316
1 768 0.7150442477876107 0.5564448530820211 0.625853090105437
1 800 0.7150442477876107 0.5564448530820211 0.625853090105437
1 832 0.7150442477876107 0.5564448530820211 0.625853090105437
1 864 0.7168141592920354 0.557034823583496 0.6269039016886445
1 896 0.7168141592920354 0.557034823583496 0.6269039016886445
1 928 0.7185840707964601 0.5588047350879207 0.6287015816485252
1 960 0.7185840707964601 0.5588047350879207 0.6287015816485252
1 992 0.7185840707964601 0.5588047350879207 0.6287015816485252
1 1024 0.7185840707964601 0.5588047350879207 0.6287015816485252
2 64 0.6115044247787611 0.5668633873501132 0.5883383202455638
2 96 0.6539823008849558 0.6059757499138031 0.6290644596586055
2 128 0.6964601769911505 0.6471683331417845 0.6709101041602659
2 160 0.715929203539823 0.6650283492318891 0.6895406965136408
2 192 0.7212389380530974 0.670043098494426 0.694699076266582
2 224 0.7309734513274336 0.6794826265180247 0.7042881638421795
2 256 0.7380530973451327 0.6873882312377887 0.7118202664265316
2 288 0.7415929203539823 0.6904855763705321 0.7151273009323443
2 320 0.7451327433628319 0.6940253993793816 0.7186716100812495
2 352 0.7451327433628319 0.6940253993793816 0.7186716100812495
2 384 0.7477876106194691 0.6966802666360188 0.7213298130842928
2 416 0.7495575221238938 0.6984501781404435 0.7231019348286224
2 448 0.7486725663716814 0.6975652223882312 0.7222158753089077
2 480 0.7495575221238938 0.6984501781404435 0.7231019348286224
2 512 0.7469026548672566 0.6957953108838064 0.7204437481448223
2 544 0.7460176991150442 0.694910355131594 0.7195576804804923
2 576 0.7424778761061946 0.6913705321227445 0.7160133823727665
2 608 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 640 0.7389380530973452 0.6881256943646323 0.7126272554879096
2 672 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 704 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 736 0.7407079646017699 0.6898956058690571 0.7143994053402157
2 768 0.7380530973451327 0.6876832164885262 0.7119783974034849
2 800 0.7380530973451327 0.6876832164885262 0.7119783974034849
2 832 0.7380530973451327 0.6876832164885262 0.7119783974034849
2 864 0.7389380530973452 0.6882731869900011 0.7127063387790727
2 896 0.7407079646017699 0.6900430984944259 0.7144784751964081
2 928 0.7424778761061946 0.6918130099988506 0.7162506006315945
2 960 0.7424778761061946 0.6918130099988506 0.7162506006315945
2 992 0.7424778761061946 0.6918130099988506 0.7162506006315945
2 1024 0.7380530973451327 0.6873882312377887 0.7118202664265316
3 64 0.6227138643067849 0.6045625023943607 0.6135039544400294
3 96 0.6731563421828908 0.6533208826571657 0.6630903077800281
3 128 0.7197640117994101 0.6990570049419607 0.7092594039932004
3 160 0.7380530973451328 0.7159717273876567 0.7268447443558818
3 192 0.741297935103245 0.7195536911466117 0.7302639855523161
3 224 0.7513274336283189 0.7295831896716853 0.7402956760387077
3 256 0.7607669616519176 0.7392439566333373 0.7498510470182278
3 288 0.7651917404129795 0.7435212427690305 0.7542008587856368
3 320 0.768731563421829 0.7470610657778801 0.7577414086915233
3 352 0.7766961651917406 0.7550256675477917 0.765707621411733
3 384 0.7787610619469029 0.7570905643029539 0.7677729303659072
3 416 0.7823008849557525 0.7606303873118033 0.7713134548679701
3 448 0.7825958702064899 0.7609253725625409 0.771608498286004
3 480 0.7828908554572273 0.7612203578132782 0.7719035416595889
3 512 0.7820058997050148 0.7603354020610659 0.7710184114054363
3 544 0.7811209439528024 0.7594504463088535 0.7701332807503245
3 576 0.7820058997050148 0.7603354020610659 0.7710184114054363
3 608 0.7820058997050148 0.7603354020610659 0.7710184114054363
3 640 0.7805309734513275 0.7590079684327473 0.769619023385166
3 672 0.7787610619469026 0.7572380569283225 0.7678487651632744
3 704 0.7761061946902655 0.7545831896716854 0.7651933748236583
3 736 0.7761061946902655 0.7545831896716854 0.7651933748236583
3 768 0.7758112094395281 0.7545831896716854 0.7650499731858795
3 800 0.7764011799410031 0.7553206527985289 0.7657158545788109
3 832 0.7764011799410031 0.7553206527985289 0.7657158545788109
3 864 0.7761061946902655 0.7550256675477914 0.7654208134333593
3 896 0.776991150442478 0.7559106233000038 0.76630593674064
3 928 0.7778761061946904 0.7567955790522162 0.7671910596614435
3 960 0.7778761061946904 0.7567955790522162 0.7671910596614435
3 992 0.7761061946902655 0.7550256675477914 0.7654208134333593
3 1024 0.7758112094395281 0.7545831896716853 0.7650499731858795


==> tables/overall.tex <==
% Please paste the tables here
9_percent\xml_test_data_after_tf_idf.json : 0.981081
9_percent\xml_train_data_after_tf_idf.json : 0.945503
60_percent\xml_test_data_after_tf_idf.json : 0.947364
60_percent\xml_train_data_after_tf_idf.json : 0.953678
70_percent\xml_test_data_after_tf_idf.json : 0.971918
70_percent\xml_train_data_after_tf_idf.json : 0.947725
100_percent\xml_test_data_after_tf_idf.json : 0.959554
100_percent\xml_train_data_after_tf_idf.json : 0.950722

9_percent\xml_test_data_after_tf_idf.json : 0.983784
9_percent\xml_train_data_after_tf_idf.json : 0.981651
60_percent\xml_test_data_after_tf_idf.json : 0.978378
60_percent\xml_train_data_after_tf_idf.json : 0.982962
70_percent\xml_test_data_after_tf_idf.json : 0.989189
70_percent\xml_train_data_after_tf_idf.json : 0.980341
100_percent\xml_test_data_after_tf_idf.json : 0.989189
100_percent\xml_train_data_after_tf_idf.json : 0.980341


Case Study:
    "desc": "Integer overflow in the crypt_raw method in the key-stretching implementation in jBCrypt before 0.4 makes it easier for remote attackers to determine cleartext values of password hashes via a brute-force attack against hashes associated with the maximum exponent.",
    "labels": [
        "com.puresoltechnologies.purifinity.server:server.ddl",
        "de.nierbeck.cassandra:Karaf-Cassandra-Embedded",
        "org.hawkular.metrics:hawkular-metrics-data-generator",
        "com.puresoltechnologies.ductiledb:ductiledb-jdbc",
        "com.puresoltechnologies.purifinity.server:global.ddl",
        "io.paradoxical:cassieq-core",
        "org.mindrot:jbcrypt"
    ]


70%占比的测试集的测试时间是2分13秒
tf-idf:26175-17846 ms (15cores)

Current works
Model this problem as a extreme multi-label learning (XML) task
Construct a dataset with labels

Limitation & Challenge:
Cannot comprehend deep-level semantic information
cannot handle zero-shot scenarios
Use only libraries’ names as labels, Current dataset does not reflect real zero-shot distribution (Java)


Resolution:
Model this task as a entity-link task to associate vuln and libraries descriptions
Construct a larger real-world dataset with zero-shot libraries  

Approach details: two stages
Efficiency: a coarse-grained tf-idf matcher to filter the candidate libraries 
Effectiveness: a fine-grained bertFNN model to identify the candidate libraries.

To the best of our knowledge, we are the first to model library identification from vulnerabilities as an entity-link task and conduct zero-shot library identification.    
We use a coarse-grained tf-idf matcher to efficiently filter the candidate libraries and a fine-grained bertFNN mode to effectively identify the candidate libraries.
We construct a new dataset that are manually labelled and validated by senior software engineers, including 2,789 Java libraries and 324 negative samples.    
We conduct a comprehensive evaluation of demonstrating detector’s effectiveness and efficiency for library identification, and generalization abilities in zero-shot libraries, boosting the average F1 score from 0.54 to 0.76 and complementing the lack labels of all Java vulnerabilities from CVE.


\begin{lstlisting}
    def expand_apostrophe(string):
    pat_is = re.compile("(it|he|she|that|this|there|here)(\'s)", re.I)
    pat_s = re.compile("(?<=[a-zA-Z])\'s")
    pat_s2 = re.compile("(?<=s)\'s?")
    pat_not = re.compile("(?<=[a-zA-Z])\'t")
    pat_would = re.compile("(?<=[a-zA-Z])\'d")
    pat_will = re.compile("(?<=[a-zA-Z])\'ll")
    pat_am = re.compile("(?<=[I|i])\'m")
    pat_are = re.compile("(?<=[a-zA-Z])\'re")
    pat_ve = re.compile("(?<=[a-zA-Z])\'ve")

    text = pat_is.sub(r"\1 is", string)
    text = re.sub(r"won't", "will not", text)
    text = pat_s.sub("", text)
    text = pat_s2.sub("", text)
    text = pat_not.sub(" not", text)
    text = pat_would.sub(" would", text)
    text = pat_will.sub(" will", text)
    text = pat_am.sub(" am", text)
    text = pat_are.sub(" are", text)
    text = pat_ve.sub(" have", text)
    text = text.replace('\'', ' ')
    return text


def remove_stopwords(tokens):
    return [w for w in tokens if not (w in stopwds)]


def cleaned_text(text):
    text = expand_apostrophe(text)
    text = re.sub(u'[^a-zA-Z]', ' ', text)
    tokens = text.lower().strip().split()
    rmstw_tokens = remove_stopwords(tokens)
    return rmstw_tokens


class PreSearch:
    def __init__(self, vul_corpus, lib_file):
        with open(lib_file, "r", encoding="utf-8") as f_lib:
            self.vul_corpus = vul_corpus
            self.lib_corpus = json.load(f_lib)
        self.lib_tokens = [item["name_tokens"] + item.get("desc_tokens", []) for item in self.lib_corpus]
        self.lib_tokens_num = np.array([len(item) + 1 for item in self.lib_tokens])
        self.lib_name_index = dict()
        for index, item in enumerate(self.lib_corpus):
            self.lib_name_index[item["name"].lower().replace(" ", "")] = (item["name"], index)

    def search(self):
        res = []
        for index, vul_info in enumerate(self.vul_corpus):
            named_entity_list = vul_info[4]
            named_entity_index = []
            desc_tokens = vul_info[3]
            desc_tokens = [x for x in desc_tokens if x not in freq_word_list]
            search_result = []
            if named_entity_list:
                tmp = set(named_entity_list)
                for x in named_entity_list:
                    tmp.update(remove_stopwords(cleaned_text(expand_apostrophe(x))))
                named_entity_list = list(tmp)
                search_result = self.search_by_name(named_entity_list)
                named_entity_index = [i for i, token in enumerate(desc_tokens) if token in named_entity_list]
            word_freq = self.gen_freq_matrix(desc_tokens)
            if not len(word_freq):
                continue
            scores = self.cal_tf_idf(word_freq, named_entity_index)
            top128 = self.get_top128(scores, search_result)
            tmp = {"cve_id": vul_info[0],
                   "top128": [x[1] for x in top128],
                   "desc": vul_info[1],
                   "labels": vul_info[2]}
            res.append(tmp)
        suffix = uuid.uuid1()
        result_file_name = "tf_idf_result_" + str(suffix) + ".json"
        with open(os.path.join("/", "clouddragonData", "bingjie", "data", result_file_name), "w", encoding="utf-8") as f:
            json.dump(res, f, indent=4)

    @staticmethod
    def get_nonzero_count(array):
        return len(array[array > 0])

    def get_top128(self, scores, search_result):
        sorted_id = sorted(range(len(scores)), key=lambda k: scores[k], reverse=True)
        search_result_id = [x[1] for x in search_result]
        tf_idf_result_id = [x for x in sorted_id[:128] if x not in search_result_id]
        top = search_result_id + tf_idf_result_id
        return [(i, self.lib_corpus[i]["name"], scores[i]) for i in top[:128]]

    def cal_tf_idf(self, word_freq, named_entity_index):
        tf = self.cal_tf(word_freq)
        idf = self.cal_idf(word_freq)
        scores = tf * idf
        row_num = np.size(scores, axis=0)
        for index in named_entity_index:
            scores[index] *= 4
            row_num += 3
        return np.sum(scores, axis=0) / row_num

    def cal_tf(self, word_freq):
        return word_freq / self.lib_tokens_num

    def cal_idf(self, word_freq):
        exist_text_count = np.zeros(word_freq.shape)
        for i in range(word_freq.shape[0]):
            exist_text_count[i, :] = self.get_nonzero_count(word_freq[i, :]) + 1
        return np.log(len(self.lib_tokens_num) / exist_text_count)

    def gen_freq_matrix(self, words):
        res = []
        for word in words:
            res.append([list(text).count(word) for text in self.lib_tokens])
        return np.array(res)

    def search_by_name(self, named_entity_list):
        res = []
        for named_entity in named_entity_list:
            if named_entity.lower().replace(" ", "") in self.lib_name_index:
                res.append(self.lib_name_index[named_entity.lower().replace(" ", "")])
        return res


def actions(partitions):
    searcher = PreSearch(partitions, lib_file)
    searcher.search()


if __name__ == "__main__":
    word_file = "word_list.txt"
    word_file = os.path.join("/", "clouddragonData", "bingjie", word_file)
    with open(word_file, "r", encoding="utf-8") as f:
        freq_word_list = f.read().split(" ")
    vul_file = "python_vul_train_before_tf_idf_2.json"
    vul_file = os.path.join("/", "clouddragonData", "bingjie", vul_file)
    with open(vul_file, "r", encoding="utf-8") as f:
        vul_corpus = json.load(f)
    vul_corpus_list = [(x.get("cve_id", None),
                        x.get("desc", None),
                        x.get("labels", None),
                        x.get("desc_tokens", None),
                        x.get("named_entity", None)) for x in vul_corpus]
    lib_file = "python_lib_file.json"
    vul_file = os.path.join("/", "clouddragonData", "bingjie", lib_file)
    app_name = 'get top128 github'
    sc = SparkSession.builder.appName(app_name).getOrCreate()
    data_df = sc.createDataFrame(vul_corpus)
    df_parts = data_df.repartition(15)
    df_parts.foreachPartition(actions)
    sc.stop()


\end{lstlisting}

maven:com.adobe.acrobat:acrobat                    1341


fastxml
  配置：Intel(R)
  Core(TM) i7-8700 CPU @ 3.20GHz 6核32G
  训练时间：200迭代次数  205.22s
  测试时间：7.58s
lightxml
  配置：Intel(R)
  Xeon(R) CPU E5-2697 v4 @ 2.30GHz
  36核256G
  用的单GPU: Tesla P100 PCIe 16GB

  训练时间：bert-base
  20epoch 1h34min5s + roberta
  20epoch 1h34min6s + xlnet
  20epoch 2h58min13s =
  6h18min48s

  测试时间：bert-base
  28.3s + roberta
  26.68s + xlnet
  73.37s = 128.35s

14: complete matching
Lacking:
9059: partial matching
  7936:2015-2022

  12716 pairs
    pair vul lib
  12716 6567 3204
  7936 3617 2443

  6567 vulnerabilities
  3204 libraries

  {
    "cve_id": "CVE-2016-4055",
    "top128": [
        "com.liferay.portal:portal-service",
        "org.apache.hive:hive-service",
        "com.liferay:com.liferay.knowledge.base.service",
        "net.winroad:wrdoclet",
        "org.apache.tomcat:el-api",
        "org.webjars.npm:moment",
        "org.webjars.bower:moment",
        "org.apache.nifi:nifi-jms-cf-service",
        "org.webjars.bower:auth0.js",
        "org.webjars:qs",
        "com.microsoft.azure.sdk.iot:iot-service-client",
        "org.apache.nifi:nifi-jms-cf-service-nar",
        "org.apache.tomcat:tomcat-catalina-jmx-remote",
        "org.webjars.bower:mapbox.js.compiled",
        "org.webjars.bower:momentjs",
        "com.wavefront:proxy",
        "com.github.tomakehurst:wiremock",
        "com.github.mtakaki:credential-storage",
        "com.automation-remarks:video-recorder-remote",
        "org.webjars.bower:plotly.js",
        "org.ops4j.pax.wicket:org.ops4j.pax.wicket.service",
        "com.github.mtakaki:credential-storage-client",
        "org.springframework.batch:spring-batch-admin-manager",
        "org.apache.karaf.kar:org.apache.karaf.kar.core",
        "org.springframework.social:spring-social-core",
        "com.linecorp.centraldogma:centraldogma-server",
        "io.pivotal.spring.cloud:spring-cloud-sso-connector",
        "org.codehaus.jackson:jackson-mapper-asl",
        "org.codehaus.jackson:jackson-mapper-lgpl",
        "com.danielflower.apprunner:app-runner",
        "org.apache.shiro:shiro-all",
        "org.apache.sling:org.apache.sling.auth.core",
        "com.rabbitmq:amqp-client",
        "com.madgag.spongycastle:bctls-jdk15on",
        "org.hudsonci.plugins:favorite",
        "bouncycastle:bcprov-jdk12",
        "bouncycastle:bcprov-jdk15",
        "bouncycastle:bcprov-jdk14",
        "bouncycastle:bcprov-jdk13",
        "org.apache.uima:uimaj-adapter-vinci",
        "org.bouncycastle:bcprov-jdk15on",
        "org.bouncycastle:bcprov-jdk16",
        "org.bouncycastle:bcprov-jdk15",
        "org.bouncycastle:bcprov-jdk14",
        "org.jvnet.hudson.plugins:repository-connector",
        "org.bouncycastle:bcprov-ext-jdk15",
        "org.bouncycastle:bcprov-ext-jdk15on",
        "org.bouncycastle:bcprov-ext-jdk14",
        "org.bouncycastle:bcprov-debug-jdk14",
        "com.typesafe.akka:akka-remote_2.13.0-M3",
        "com.typesafe.akka:akka-remote_2.11",
        "com.typesafe.akka:akka-remote_2.12",
        "org.awake-file:awake-file",
        "org.bouncycastle:bcprov-ext-debug-jdk15on",
        "org.bouncycastle:bcprov-ext-debug-jdk14",
        "bouncycastle:bcprov-jdk16",
        "org.bouncycastle:bcprov-ext-jdk16",
        "org.bouncycastle:bcprov-jdk15+",
        "org.bouncycastle:bcprov-debug-jdk15on",
        "org.apache.xmlrpc:xmlrpc",
        "pmd:pmd",
        "io.advantageous.qbit:qbit-vertx",
        "com.hazelcast:hazelcast",
        "org.codehaus.groovy:groovy-all",
        "com.eclipsesource.jaxrs:swagger-all",
        "org.mortbay.jasper:apache-jsp",
        "org.apache.taglibs:taglibs-standard",
        "com.frightanic:open-data-smn",
        "com.alibaba:fastjson",
        "io.spray:spray-json_2.11",
        "org.apache.ranger:ranger-kafka-plugin",
        "org.jvnet.hudson.plugins:copy-to-slave",
        "com.github.sakserv:hadoop-mini-clusters-hbase",
        "org.eclipse.rdf4j:rdf4j-util",
        "org.wildfly:wildfly-iiop-openjdk",
        "org.sonarsource.sonarqube:sonar-scanner-engine-shaded",
        "net.sourceforge.jmatio:jmatio",
        "org.apache.poi:poi",
        "io.spray:spray-json_2.12.0-M5",
        "com.github.axet:zip4j",
        "org.apache.shiro:shiro-web",
        "com.fasterxml.jackson.datatype:jackson-datatype-jsr310",
        "mysql:mysql-connector-java",
        "org.richfaces:richfaces-a4j",
        "org.bouncycastle:bctsp-jdk14",
        "org.apache.nifi:nifi-framework-core",
        "org.apache.opennlp:opennlp-uima",
        "org.apache.cassandra:cassandra-all",
        "org.apache.hbase:hbase-client",
        "org.elasticsearch:elasticsearch",
        "org.jasig.cas:cas-server-support-ldap",
        "org.apache.camel:camel-xstream",
        "com.orientechnologies:orientdb-server",
        "org.apache.xmlrpc:xmlrpc-client",
        "org.apache.brooklyn:brooklyn",
        "com.typesafe.play:play_2.12",
        "com.sparkjava:spark-core",
        "org.springframework:spring-core",
        "com.jason-goodwin:authentikat-jwt_2.10",
        "org.apache.brooklyn:brooklyn-jsgui",
        "org.apache.camel:camel-castor",
        "org.cloudfoundry:cloudfoundry-client",
        "com.elastisys.scale:cloudadapters.openstack",
        "taglibs:standard",
        "org.mindrot:jbcrypt",
        "org.webjars.bower:bootstrap",
        "org.idpf:epubcheck",
        "org.onosproject:onlab-stc",
        "org.apache.camel:camel-spark-rest",
        "org.apache.kafka:kafka_2.11",
        "org.springframework.integration:spring-integration-xml",
        "com.adobe.xmp:xmpcore",
        "com.iveely:com.iveely.framework",
        "org.webjars.bower:pouchdb",
        "org.apache.syncope.core:syncope-core-provisioning-java",
        "org.igniterealtime.openfire:xmppserver",
        "org.keycloak:keycloak-spring-security-adapter",
        "org.apache.flink:flink-shaded-curator-recipes",
        "org.ow2.jonas:jonas-webservices-axis",
        "org.graniteds:granite-server-beanvalidation",
        "org.bouncycastle:bctls-jdk15on",
        "org.apache.cxf:cxf-rt-rs-extension-providers",
        "org.apache.uima:uimaj-tools",
        "org.keycloak:keycloak-services",
        "org.webjars.npm:lodash",
        "org.apache.spark:spark-launcher_2.10",
        "org.webjars.npm:semver",
        "commons-httpclient:commons-httpclient"
    ],
    "desc": "The duration function in the moment package before 2.11.2 for Node.js allows remote attackers to cause a denial of service (CPU consumption) via a long string, aka a \"regular expression Denial of Service (ReDoS).\"",
    "labels": [
        "org.webjars.npm:moment",
        "org.webjars.bower:moment",
        "org.webjars.bower:momentjs",
        "org.webjars:momentjs"
    ]
},

9047	12703	63890bd37cfb3d163d475b98	CVE-2018-18511	maven:org.webjars.npm:canvas	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9048	12704	638da834050e3e3db53f13f5	CVE-2021-37533	maven:commons-net:commons-net	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9049	12705	638daf39050e3e3db53f142e	CVE-2021-21693	maven:org.jenkins-ci.main:jenkins-core	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9050	12707	638dbdc9050e3e3db53f1430	CVE-2022-1471	maven:org.yaml:snakeyaml	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9051	12708	638dc2d4050e3e3db53f1431	CVE-2022-21126	maven:com.github.samtools:htsjdk_2.11	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9052	12709	638dc2d4050e3e3db53f1432	CVE-2022-21126	maven:com.github.samtools:htsjdk	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9053	12710	638dc319050e3e3db53f1433	CVE-2022-24999	maven:org.webjars.bower:qs	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9054	12711	638dc7d3050e3e3db53f1434	CVE-2022-46366	maven:org.apache.tapestry:tapestry-core	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9055	12712	638dc7d3050e3e3db53f1435	CVE-2022-46366	maven:org.apache.tapestry:tapestry-framework	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9056	12713	638dd24a050e3e3db53f1436	CVE-2022-41404	maven:org.webjars.npm:node-fetch	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9057	12714	638dd461050e3e3db53f1437	CVE-2022-45933	maven:org.webjars:kube	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend
9058	12715	638dd781050e3e3db53f1438	CVE-2022-41965	maven:org.opencastproject:opencast-kernel	VulLibMatchBasedOnEntityLink	com.huawei.fossbotkbserver.model.vul.VulRecommend



Total vulns
2    122681
0     57657
1     24167

Java vulns:
2    1884
0    1314
1     419

Training Dataset:
2    1961
1     651
0     177

组内平均距离0.6422015875479155
全部平均距离0.45375659832711446
分位数：0.9754042227109962
平均有 78.8个相似度高于0.6422的（3204个lib）

maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-client
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-core
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-web-console
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-http
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-all
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-mqtt
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:artemis-web
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-broker
maven:org.apache.activemq:activemq-web maven:org.apache.activemq:activemq-jaas

maven:org.apache.tomcat.embed:tomcat-embed-core maven:org.apache.tomcat.embed:tomcat-embed-jasper
maven:org.apache.tomcat.embed:tomcat-embed-core maven:org.apache.tomcat.embed:tomcat-embed-websocket
maven:org.apache.tomcat.embed:tomcat-embed-core maven:org.apache.tomcat.embed:tomcat-embed-el

top64:67.41\%
top128:75.40\%
top256:87.09\%
top512:90.01\%
top1024:92.57\%
top2048:94.02\%




\begin{table}[]
\begin{tabular}{lllllllllllllll}
\cline{1-4}
                                             & Zero-shot   percent & 模型             & Train(漏洞) & Test正样本(漏洞) & Top1  &        &       & Top2  &        &       & Top3  &        &       & 模型    \\ \cline{1-4}
                                             &                     &                &           &             & Prec  & Recall & F1    & Prec  & Recall & F1    & Prec  & Recall & F1    &       \\
OurData   0.1                                & 0                   & Fast XML       & 1668      & 657         & 0.616 & 0.473  & 0.535 & 0.427 & 0.594  & 0.497 & 0.329 & 0.647  & 0.436 & fx模型1 \\
                                             &                     & Light   XML    & 1668      & 657         & 0.712 & 0.567  & 0.632 & 0.467 & 0.673  & 0.552 & 0.351 & 0.725  & 0.473 & lx模型2 \\ \cline{1-4}
                                             &                     & Bert   FNN@128 & 1860      & 657         & 0.678 & 0.536  & 0.599 & 0.427 & 0.627  & 0.508 & 0.316 & 0.665  & 0.428 & 模型1   \\
                                             &                     & Bert   FNN@512 & 1860      & 657         & 0.72  & 0.575  & 0.639 & 0.46  & 0.69   & 0.552 & 0.349 & 0.753  & 0.477 & 模型1   \\ \cline{1-4}
                                             & 29.3                & Fast XML       & 1668      & 1121        & 0.413 & 0.294  & 0.343 & 0.289 & 0.372  & 0.325 & 0.225 & 0.408  & 0.29  & fx模型1 \\
                                             &                     & Light   XML    & 1668      & 1121        & 0.444 & 0.328  & 0.377 & 0.295 & 0.398  & 0.339 & 0.225 & 0.434  & 0.297 & lx模型1 \\
                                             &                     & Bert   FNN@128 & 1860      & 1121        & 0.619 & 0.467  & 0.53  & 0.402 & 0.565  & 0.470 & 0.297 & 0.600  & 0.398 & 模型1   \\
                                             &                     & Bert   FNN@512 & 1860      & 1121        & 0.629 & 0.477  & 0.542 & 0.413 & 0.59   & 0.486 & 0.313 & 0.645  & 0.421 & 模型1   \\
                                             & 100                 & Fast XML       & 1668      & 329         & 0     & 0      & 0     & 0     & 0      & 0     & 0     & 0      & 0     & fx模型1 \\
                                             &                     & Light   XML    & 1668      & 329         & 0     & 0      & 0     & 0     & 0      & 0     & 0     & 0      & 0     & lx模型3 \\
                                             &                     & Bert   FNN@128 & 1860      & 329         & 0.492 & 0.428  & 0.458 & 0.319 & 0.541  & 0.401 & 0.224 & 0.559  & 0.320 & 模型1   \\
                                             &                     & Bert   FNN@512 & 1860      & 329         & 0.453 & 0.386  & 0.417 & 0.3   & 0.504  & 0.376 & 0.217 & 0.543  & 0.31  & 模型1   \\
\textbackslash{}rowcolor{[}HTML{]}\{92D050\} &                     &                &           &             &       &        &       &       &        &       &       &        &       &       \\
OurData   0.1 mock                           & 0                   & Fast XML       & 1789      & 601         & 0.636 & 0.501  & 0.56  & 0.444 & 0.63   & 0.521 & 0.336 & 0.683  & 0.45  & fx模型2 \\
                                             &                     & Light   XML    & 1789      & 601         & 0.75  & 0.615  & 0.676 & 0.493 & 0.732  & 0.589 & 0.361 & 0.77   & 0.492 & lx模型4 \\
                                             &                     & Bert FNN       & 1789      & 601         & 0.650 & 0.520  & 0.578 & 0.406 & 0.596  & 0.483 & 0.294 & 0.624  & 0.400 & 模型2   \\
                                             & 100                 & Fast XML       & 1748      & 642         & 0     & 0      & 0     & 0     & 0      & 0     & 0     & 0      & 0     & fx模型3 \\
                                             &                     & Light   XML    & 1748      & 642         & 0     & 0      & 0     & 0     & 0      & 0     & 0     & 0      & 0     & lx模型5 \\
                                             &                     & Bert FNN       & 1748      & 642         & 0.390 & 0.353  & 0.371 & 0.242 & 0.421  & 0.308 & 0.182 & 0.463  & 0.261 & 模型3   \\
\textbackslash{}rowcolor{[}HTML{]}\{92D050\} &                     &                &           &             &       &        &       &       &        &       &       &        &       &       \\
论文数据集                                        & 0                   & Fast XML       &           &             &       &        &       &       &        &       &       &        &       &       \\
                                             &                     & Light   XML    &           &             &       &        &       &       &        &       &       &        &       &       \\
                                             &                     & Bert FNN       &           &             &       &        &       &       &        &       &       &        &       &       \\
                                             & 29.3                & Fast XML       &           &             &       &        &       &       &        &       &       &        &       &       \\
                                             &                     & Light   XML    &           &             &       &        &       &       &        &       &       &        &       &       \\
                                             &                     & Bert FNN       &           &             &       &        &       &       &        &       &       &        &       &       \\
                                             & 100                 & Fast XML       &           &             &       &        &       &       &        &       &       &        &       &       \\
                                             &                     & Light   XML    &           &             &       &        &       &       &        &       &       &        &       &       \\

NER:
training: 2196 vuln descriptions
testing: 548 vuln descriptions

precision: 0.9285
recall: 0.9616
F1: 9448

Input: Vuln descriptions 
Output: Token Labels
                                             
                                             &                     & Bert FNN       &           &             &       &        &       &       &        &       &       &        &       &      
\end{tabular}
\end{table}



cve_id	component_name
CVE-2022-3471	maven:org.apache.storm:sql
CVE-2022-3471	maven:cn.sexycode:my-sql
CVE-2022-3471	maven:dev.rudiments:sql
CVE-2022-3471	maven:xyz.cofe:sql
CVE-2022-3471	maven:taglibs:sql
CVE-2022-3471	maven:commons-sql:commons-sql
CVE-2022-3471	maven:org.cloudhoist:php
CVE-2022-3471	maven:net.bookrain:file
CVE-2022-3471	maven:com.daioware:file
CVE-2022-3471	maven:cocoon:cocoon-php
CVE-2022-0583	maven:io.americanexpress:service
CVE-2022-1354	maven:net.bookrain:file
CVE-2022-1354	maven:com.facebook:slice
CVE-2022-3324	maven:org.eclipse.milo:stack-core
CVE-2022-0175	maven:slide:kernel
CVE-2022-0175	maven:com.datathings:greycat-memory
CVE-2022-1319	maven:io.undertow:undertow-core
CVE-2022-1319	maven:io.undertow:undertow-parent
CVE-2022-1319	maven:io.undertow:undertow-examples
CVE-2022-1319	maven:taglibs:response
CVE-2022-1319	maven:io.undertow:undertow-benchmarks
CVE-2022-1319	maven:io.undertow:undertow-servlet
CVE-2022-1319	maven:io.undertow:undertow-dist
CVE-2022-1319	maven:io.undertow:undertow-jsp
CVE-2022-3473	maven:org.apache.storm:sql
CVE-2022-3473	maven:cn.sexycode:my-sql
CVE-2022-3473	maven:commons-sql:commons-sql
CVE-2022-3473	maven:dev.rudiments:sql
CVE-2022-3473	maven:xyz.cofe:sql
CVE-2022-3473	maven:org.cloudhoist:php
CVE-2022-3473	maven:taglibs:sql
CVE-2022-3473	maven:ru.hnau:possible
CVE-2022-3473	maven:maven:wagon-file
CVE-2022-3473	maven:cocoon:cocoon-php
CVE-2022-3470	maven:org.apache.storm:sql
CVE-2022-3470	maven:cn.sexycode:my-sql
CVE-2022-3470	maven:taglibs:sql
CVE-2022-3470	maven:commons-sql:commons-sql
CVE-2022-3470	maven:dev.rudiments:sql
CVE-2022-3470	maven:xyz.cofe:sql
CVE-2022-3470	maven:org.cloudhoist:php
CVE-2022-3470	maven:cocoon:cocoon-php
CVE-2022-3470	maven:ru.hnau:possible
CVE-2022-3470	maven:net.bookrain:file
CVE-2022-3504	maven:taglibs:sql
CVE-2022-3504	maven:xyz.cofe:sql
CVE-2022-3504	maven:dev.rudiments:sql
CVE-2022-3504	maven:commons-sql:commons-sql
CVE-2022-3504	maven:org.cloudhoist:php
CVE-2022-3504	maven:cocoon:cocoon-php
CVE-2022-3504	maven:net.bookrain:file
CVE-2022-3504	maven:com.daioware:file
CVE-2022-3504	maven:org.sql2o:sql2o
CVE-2022-3504	maven:com.ruijc:id
CVE-2022-0586	maven:io.americanexpress:service
CVE-2022-0581	maven:io.americanexpress:service
CVE-2022-1734	maven:sh.almond:kernel_2.11
CVE-2022-1734	maven:sh.almond:kernel_2.12
CVE-2022-1734	maven:sh.almond:kernel_2.13
CVE-2022-1734	maven:slide:kernel
CVE-2022-1734	maven:ru.tinkoff.core:core-nfc
CVE-2022-1734	maven:sh.almond:echo-kernel_2.11
CVE-2022-1734	maven:sh.almond:echo-kernel_2.12
CVE-2022-3171	maven:jetty:embedded
CVE-2022-3171	maven:net.spals.shaded:protobuf-java
CVE-2022-3171	maven:swt:forms
CVE-2022-3171	maven:io.swaydb:embedded_2.11
CVE-2022-3171	maven:org.zapodot:embedded-db-core
CVE-2022-3171	maven:io.swaydb:embedded_2.12
CVE-2022-3171	maven:org.nd4j:protobuf
CVE-2022-3171	maven:vip.isass:super-core-protobuf
CVE-2022-3171	maven:org.postgresql:pgjdbc-versions
CVE-2022-3171	maven:org.javastro:bom
CVE-2022-3495	maven:taglibs:sql
CVE-2022-3495	maven:commons-sql:commons-sql
CVE-2022-3495	maven:org.cloudhoist:php
CVE-2022-3495	maven:cocoon:cocoon-php
CVE-2022-3495	maven:org.sql2o:sql2o
CVE-2022-3495	maven:org.netbeans.cluster:php
CVE-2022-3495	maven:org.jenkins-ci.plugins:google-login
CVE-2022-1355	maven:org.eclipse.milo:stack-core
CVE-2022-1355	maven:org.eclipse.milo:stack-client
CVE-2022-3296	maven:org.eclipse.milo:stack-core
CVE-2022-3465	maven:net.bookrain:file
CVE-2022-3465	maven:maven:wagon-file
CVE-2022-3503	maven:io.markdom:handler
CVE-2022-3503	maven:net.darkmist.alib:handler
CVE-2022-3503	maven:net.bookrain:system
CVE-2022-3503	maven:org.tinygroup:order
CVE-2022-3503	maven:org.randombits.supplier:supplier-core
CVE-2022-3503	maven:org.aperteworkflow:scripting
CVE-2022-3503	maven:org.tuxdevelop:address-migrator
CVE-2022-3503	maven:io.jenkins.plugins:oversecured
CVE-2022-0585	maven:io.americanexpress:service
CVE-2022-2953	maven:org.marketcetera:fix-core
CVE-2022-2953	maven:io.americanexpress:service
CVE-2022-2953	maven:com.vesoft:tools
CVE-2022-2953	maven:maven:wagon-file
CVE-2022-2953	maven:org.marketcetera:fix-initiator
CVE-2022-2953	maven:net.bookrain:file
CVE-2022-2953	maven:org.bekit:service
CVE-2022-2953	maven:com.daioware:file
CVE-2022-2953	maven:com.intersult:jpa-fix
CVE-2022-2953	maven:com.csicit.ace:file
CVE-2022-3472	maven:org.apache.storm:sql
CVE-2022-3472	maven:cn.sexycode:my-sql
CVE-2022-3472	maven:dev.rudiments:sql
CVE-2022-3472	maven:taglibs:sql
CVE-2022-3472	maven:xyz.cofe:sql
CVE-2022-3472	maven:commons-sql:commons-sql
CVE-2022-3472	maven:org.cloudhoist:php
CVE-2022-3472	maven:net.bookrain:file
CVE-2022-3472	maven:com.daioware:file
CVE-2022-3472	maven:cocoon:cocoon-php
CVE-2022-2963	maven:jetty:jasper-compiler
CVE-2022-2963	maven:tomcat:jasper-compiler
CVE-2022-2963	maven:tomcat:jasper
CVE-2022-2963	maven:axis2:security
CVE-2022-0582	maven:io.americanexpress:service
CVE-2022-1706	maven:org.brillien:ignition
CVE-2022-1706	maven:io.confound:config
CVE-2022-1706	maven:io.scalecube:config
CVE-2022-1706	maven:com.jpmorgan.quorum:config
CVE-2022-1706	maven:io.swaydb:configs_2.11
CVE-2022-1706	maven:com.trib3:config
CVE-2022-1706	maven:com.vii.brillien:ignition
CVE-2022-1706	maven:io.swaydb:configs_2.12
CVE-2022-1706	maven:io.swaydb:configs_2.13
CVE-2022-1706	maven:com.frontegg:config
CVE-2022-3502	maven:io.markdom:handler
CVE-2022-3502	maven:io.netty:netty-handler
CVE-2022-3502	maven:net.darkmist.alib:handler
CVE-2022-3502	maven:ru.hnau:possible
CVE-2022-3502	maven:io.servicecomb:handler-bizkeeper
CVE-2022-3502	maven:io.servicecomb:handler-loadbalance
CVE-2022-3505	maven:taglibs:page-doc
CVE-2022-3505	maven:org.cloudhoist:php
CVE-2022-3505	maven:cocoon:cocoon-php
CVE-2022-3505	maven:cn.sexycode:springo-sms
CVE-2022-3505	maven:ru.hnau:possible
CVE-2022-3505	maven:com.daioware:file
CVE-2022-3505	maven:net.bookrain:file
CVE-2022-3505	maven:taglibs:page
CVE-2022-3505	maven:tech.aegean:nirvana-page
CVE-2022-3505	maven:org.netbeans.cluster:php
CVE-2022-2805	maven:org.ovirt.engine.sdk:ovirt-engine-sdk-java
CVE-2022-2256	maven:org.keycloak:keycloak-services
CVE-2022-2256	maven:org.keycloak:keycloak-core
CVE-2022-2421	maven:org.webjars.npm:socket.io
CVE-2022-2421	maven:org.webjars.bower:socket.io
CVE-2022-2047	maven:org.eclipse.jetty:jetty-http
CVE-2022-2047	maven:org.eclipse.jetty:jetty-util
CVE-2022-2047	maven:org.eclipse.jetty:jetty-server
CVE-2022-2048	maven:org.eclipse.jetty:jetty-server
CVE-2022-2048	maven:org.eclipse.jetty:jetty-http
CVE-2022-2668	maven:org.keycloak:keycloak-services
CVE-2022-2668	maven:org.keycloak:keycloak-core
CVE-2022-1552	maven:org.postgresql:postgresql
CVE-2022-1552	maven:postgresql:postgresql
CVE-2022-2764	maven:io.undertow:undertow-core
CVE-2022-3952	maven:com.manydesigns:portofino-core
CVE-2022-3952	maven:com.manydesigns:portofino-cryptography
CVE-2022-3964	maven:net.bramp.ffmpeg:ffmpeg
CVE-2022-1259	maven:io.undertow:undertow-core
CVE-2022-3873	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-0084	maven:org.jboss.xnio:xnio-all
CVE-2022-0636	maven:wiki.thin:installer
CVE-2022-0613	maven:org.webjars.npm:urijs
CVE-2022-0613	maven:org.webjars.bower:urijs
CVE-2022-0722	maven:org.webjars.npm:url-parse
CVE-2022-0806	maven:org.webjars.npm:canvas
CVE-2022-0866	maven:org.jboss.as:jboss-as-ejb3
CVE-2022-0265	maven:com.hazelcast:hazelcast-all
CVE-2022-0225	maven:org.keycloak:keycloak-services
CVE-2022-0225	maven:org.keycloak:keycloak-core
CVE-2022-0355	maven:org.webjars.bower:npm
CVE-2022-0403	maven:org.webjars.bower:elfinder
CVE-2022-0552	maven:io.netty:netty-codec-http
CVE-2022-0552	maven:io.netty:netty
CVE-2022-0552	maven:io.netty:netty-all
CVE-2022-0536	maven:org.webjars.bower:npm
CVE-2022-1217	maven:org.webjars:tinymce
CVE-2022-1217	maven:org.webjars.bower:tinymce
CVE-2022-1385	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-1379	maven:net.sourceforge.plantuml:plantuml
CVE-2022-1982	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-1575	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1548	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-1767	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1730	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1727	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1722	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1723	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1721	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1713	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1711	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1799	maven:org.microg.gms:play-services-basement
CVE-2022-1784	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1774	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1815	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-2401	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-2408	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-2576	maven:org.eclipse.californium:californium-core
CVE-2022-2576	maven:org.eclipse.californium:parent
CVE-2022-2053	maven:io.undertow:undertow-core
CVE-2022-2015	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-2014	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-2191	maven:org.eclipse.jetty:jetty-server
CVE-2022-2191	maven:org.eclipse.jetty:jetty-util
CVE-2022-2218	maven:org.webjars.npm:url-parse
CVE-2022-2838	maven:xerces:xercesImpl
CVE-2022-4044	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-4045	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-4019	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-2625	maven:postgresql:postgresql
CVE-2022-3065	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-3148	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-3147	maven:org.jenkins-ci.plugins:mattermost
CVE-2022-3138	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-3133	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-3127	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-3193	maven:org.ovirt.engine.sdk:ovirt-engine-sdk-java
CVE-2022-3224	maven:org.webjars.npm:url-parse
CVE-2022-3223	maven:org.webjars.bowergithub.jgraph:drawio
CVE-2022-1471	maven:org.yaml:snakeyaml


==> tables/tfidf.tex <==
k, ws = 128, 128
for k in [1,2,3,4,64, 128, 256, 512, 1024, 2048]:
    ws = k
    res = [modified_metrics(item, k) for item in tests_ner_only if modified_metrics(item, k) != None]
    ps, rs, fs = [v[0] for v in res], [v[1] for v in res], [v[2] for v in res]
    print(sum(ps) / len(ps), sum(rs) / len(rs), f1_score(sum(ps) / len(ps), sum(rs) / len(rs)))


0.0017699115044247787 0.0005899705014749262 0.0008849557522123895
0.0008849557522123894 0.0005899705014749262 0.0007079646017699115
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262
0.0005899705014749262 0.0005899705014749262 0.0005899705014749262

k, ws = 128, 128
for k in [1,2,3,4,64, 128, 256, 512, 1024, 2048]:
    ws = k
    res = [modified_metrics(item, k) for item in tests_ner_0 if modified_metrics(item, k) != None]
    ps, rs, fs = [v[0] for v in res], [v[1] for v in res], [v[2] for v in res]
    print(sum(ps) / len(ps), sum(rs) / len(rs), f1_score(sum(ps) / len(ps), sum(rs) / len(rs)))
    
0.1168141592920354 0.08351032448377582 0.09739386981468186
0.13982300884955753 0.1300884955752212 0.13478021180908167
0.17699115044247782 0.17262402788951461 0.1747803138064372
0.19070796460176986 0.18914320193081255 0.18992236031684132
0.49907156265563335 0.49907156265563335 0.49907156265563335
0.6039704248553805 0.6039704248553805 0.6039704248553805
0.6886118453817569 0.6886118453817569 0.6886118453817569
0.7926498869861702 0.7926498869861702 0.7926498869861702
0.8655723480059763 0.8655723480059763 0.8655723480059763
0.9139338390223346 0.9139338390223346 0.9139338390223346

k, ws = 128, 128
for k in [1,2,3,4, 64, 128, 256, 512, 1024, 2048]:
    ws = k
    res = [modified_metrics(item, k) for item in tests_ner_4 if modified_metrics(item, k) != None]
    ps, rs, fs = [v[0] for v in res], [v[1] for v in res], [v[2] for v in res]
    print(sum(ps) / len(ps), sum(rs) / len(rs), f1_score(sum(ps) / len(ps), sum(rs) / len(rs)))

    
0.18938053097345134 0.13595870206489674 0.15828359184996593
0.22920353982300884 0.211740412979351 0.2201261719092263
0.2663716814159291 0.25980691874497175 0.26304834810244065
0.2823008849557522 0.27932230011876025 0.28080369403175737
0.6687196873922537 0.6687196873922537 0.6687196873922537
0.7863967743171284 0.7863967743171284 0.7863967743171284
0.8527952725740339 0.8527952725740339 0.8527952725740339
0.8912621154656553 0.8912621154656553 0.8912621154656554
0.9120754319426885 0.9120754319426885 0.9120754319426885
0.9332258744205645 0.9332258744205645 0.9332258744205645

k, ws = 128, 128
for k in [1,2,3,4, 64, 128, 256, 512, 1024, 2048]:
    ws = k
    res = [modified_metrics(item, k) for item in tests_ner_100 if modified_metrics(item, k) != None]
    ps, rs, fs = [v[0] for v in res], [v[1] for v in res], [v[2] for v in res]
    print(sum(ps) / len(ps), sum(rs) / len(rs), f1_score(sum(ps) / len(ps), sum(rs) / len(rs)))
    
0.1911504424778761 0.1347787610619469 0.15808966814759992
0.2176991150442478 0.2009144542772861 0.20897028716318392
0.2501474926253687 0.24426119603110746 0.24716930399784887
0.2687315634218289 0.26598896678542694 0.26735323167599134
0.6527609853273572 0.6527609853273572 0.6527609853273572
0.7736011186453666 0.7736011186453666 0.7736011186453666
0.8373085469103169 0.8373085469103169 0.8373085469103169
0.8832090181205225 0.8832090181205225 0.8832090181205225
0.9015149599662873 0.9015149599662873 0.9015149599662873
0.9133143699957857 0.9133143699957857 0.9133143699957857

